A Proof of the Marmi-Moussa-Yoccoz conjecture for rotation numbers of high type

Marmi Moussa and Yoccoz conjectured that some error function Upsilon, related to the approximation of the size of Siegel disk by some arithmetic function of the rotation number theta, is a Holder continuous function of theta with exponent 1/2. Using the renormalization invariant class of Inou and Shishikura, we prove this conjecture for the restriction of Upsilon to a class of high type numbers.

==> section5__old_.tex <==
\section{H\"older}\label{sec:arn}

\subsection{Introduction}\label{subsec:map}

We continue to use the Riemannian metric $ds=\bigl|\log|x|\bigr| |dx|$ on the interval $[-1/2,1/2]$. 
The distance with respect to this metric between two points $x,y\in[-1/2,1/2]$ will be denoted $d_{\log}(x,y)$. 
The length of $[-1/2,1/2]$ for this metric is finite (it is equal to $1+\log 2$). 
This distance is H\"older continuous with respect to the Euclidean distance, for any exponent in $(0,1)$ 
(see Section~\ref{sss:bads}).
%By Cauchy-Scwharz, $ \int_{x}^{y} \bigl|\log|x|\bigr|dx \leq \sqrt{\int_{x}^{y}dx}\sqrt{\int_{x}^{y}\bigl|\log|x|\bigr|^2dx}$ where $ M_0=\sqrt{\int_{-1/2}^{1/2}\bigl|\log|x|\bigr|^2dx }<+\infty$ hence\footnote{The distance has in fact a modulus of continuity with respect to the Euclidean distance that is better than $d$-H\"older for all exponent $d\in\R$ with $0<d<1$.}
%\[d_{\log}(x,y) \leq M_0 |x-y|^{1/2} 
%.\]

Recall our notations: $\IS$ is (a big enough subset of) the Inou-Shishikura class. Maps $f\in\IS$ have rotation number $0$: $f(0)=0$ and $f'(0)=1$. Given a holomorphic map $f$ whose domain contains $0$, fixing $0$, and with $f'(0)\neq 0$, we denote
\[f = f_0 \circ R_{\alpha(f)}\]
with $f_0'(0)=1$ and
\[R_{\theta}(z)=e^{2\pi i \theta} z.\]
With the notation of Sections~\ref{sec:prelim} and~\ref{S:lipschitz}, $f_0 = \pi(f)$.
For $A\subset \R$, $\IS_{A}$ is the set of maps $f$ with $f_0\in\IS$ and $\alpha(f)\in A$.

The renormalization $\cal R(f)$ was defined in Section~\ref{sec:prelim} for $\alpha(f)$ small and positive, more precisely for all $f\in\IS_\alpha \cup \{P_\alpha\}$ with $\alpha\in(0,\ga_*]$. Let us extend $\cal R(f)$ to maps with $\alpha\in[-\ga_*,0)$ as follows: let $s(z)=\ov{z}$; let us shorten $s\circ f\circ s^{-1}$ as $sfs^{-1}$ then $\alpha(sfs^{-1}) = -\alpha(f)\in (0,\ga_*]$; let then $\cal R(f)= \cal R(s f s^{-1})$.
Let us denote $\cal R_0(f) = (\cal R(f))_0$, so that whenever $\alpha(f)\in [-\ga_*,0)\cup(0,\ga_*]$:
\[\cal R(f) = \cal R_0(f) \circ R_{1/|\alpha(f)|}.\]

Recall that the set $\HT_N$ is the set of irrational numbers whose modified continued fraction entries are all $\geq N$, and that $\IS_N := \IS_{\HT_N}$.
Note that for $N\geq 1/\ga_*$, $\HT_N\subset A$ with $A=[-\ga_*,0)\cup(0,\ga_*]$, and that maps $f$ in $\IS_N$ or in $\setof{P_\alpha}{\alpha\in\HT_N}$ are infinitely renormalizable (for the renormalization $\cal R$ extended as above to rotation numbers in $A$): $\cal R^n(f)$ is defined.

Assume a distance function $d_T(f_0,g_0)$ has been defined\footnote{The subscript $T$ stands for Teichmüller, but our proof is valid for any metric with the required properties stated here.} over $\IS_0$, has been extended to $\IS_\R$ as follows:
\[d_{\log}(f,g)=d_{\log}(\alpha(f),\alpha(g))+d_T(f_0,g_0)\]
and that the following holds:
\[f\in\IS_N \mapsto C(f) = \Upsilon(f)-|\alpha(f)|\Upsilon(\cal R(f))\]
is bounded and is Lipschitizan over $\IS_N \cap [-1/2,1/2]$ with respect to the metric $d_{\log}$,
\[\alpha\in\HT_N \mapsto C(\alpha) = \Upsilon(P_\alpha)-|\alpha|\Upsilon(\cal R(P_\alpha))\]
too. Assume that the transversal part of renormalization is Lipschitizan over $\IS_N$ with respect to the metric $d_{\log}$, and transversally contracting (see below). Assume also that $\Upsilon$ is bounded over $\IS_N$ (in \cite{BC04} it has been proved that $\Upsilon$ is bounded over $\Pol_\R$).
This sums up as follows: 
\begin{enumerate}\setlength{\itemsep}{.5ex}
\item[.] $\forall f,g\in\cal IS_N$:
\item\label{item:it1} $\Upsilon(f)\leq K_0$
\item\label{item:it2} $|C(f)-C(g)| \leq K_1 d_{\log}(f,g)$
\item\label{item:it3} $|C(f)|\leq K_3$
\item\label{item:it4} If $\alpha(f)$ and $\alpha(g)$ have the same sign, then\\
    $d_T(\cal R_0(f),\cal R_0(g)) \leq  \lambda d_T(f_0,g_0) + K_2 d_{\log}(\alpha(f),\alpha(g))$
\item\label{item:it5} $\lambda<1$
\item[.] $\forall \alpha,\beta \in (-1/N,0)\cup(0,1/N)$:
\item\label{item:it6} $|C(P_\alpha)-C(P_\beta)| \leq K_1 d_{\log}(\alpha,\beta)$
\item\label{item:it7} $|C(P_\alpha)|\leq K_3$
\item\label{item:it8} If $\alpha$ and $\beta$ have the same sign, then\\ 
    $d_T(\cal R_0(P_\alpha), \cal R_0(P_\beta)) \leq K_2 d_{\log}(\alpha,\beta)$
\end{enumerate}

Hypothesis~\ref{item:it1} has been proved in Proposition~\ref{P:Uniformly-bounded}.
Hypothesis~\ref{item:it3} and ~\ref{item:it7} follow from Proposition~\ref{P:Uniformly-bounded} and the 
definition of $C(f)$ and $C(P_\ga)$.
Hypotheses~\ref{item:it4},~\ref{item:it5}, and ~\ref{item:it8} have been proved in Proposition~\ref{P:contracting}.
Hypotheses~\ref{item:it2} and ~\ref{item:it6} have been proved in Proposition~\ref{P:Lipschitz} in the particular case when $\alpha(f)$ and $\alpha(g)$ are both positive.
%
\begin{proof}[Proof of Hypotheses~\ref{item:it2} and ~\ref{item:it6}]
The case when $\alpha(f)$ and $\alpha(g)$ are both negative follows at once from the case when they are both positive since $C(f)=C(s f s^{-1})$.
For the case when $\alpha(f)$ and $\alpha(g)$ have opposite sign, let us assume $\alpha(f)<0<\alpha(g)$ (the other case follows by permuting $f$ and $g$).
For Hypothesis~\ref{item:it6}, it is also very simple because $s P_\alpha s^{-1} = P_{-\alpha}$ hence $|C(P_\alpha)-C(P_\beta)| = |C(P_{-\alpha})-C(P_\beta)| \leq K_1 d_{\log}(-\alpha,\beta) < K_1 d_{\log}(\alpha,\beta)$.\footnote{For maps in $\IS_{N}$, we cannot use this trick because there is also the term $d_T(f_0,g_0)$ to take into account, and $d_T((s f s^{-1})_0,g_0) = d_T(sf_0 s^{-1},g_0)$ could be much bigger than $d_T(f_0,g_0)$, even when $\alpha(f)$ and $\alpha(g)$ are small.}
%: just imagine taking $g_0=f_0$ for an $f_0$ such that $sf_0 s^{-1} \neq f_0$.}
%We will first prove that $C(f_0 \circ R_\alpha)$ has a limit when $f_0$ is fixed and $\alpha\tend 0$ from the right and from the left, and that these two limits are the same. 
%The fact that the two limits exist can be deduced for instance from the same signe case of Hypothesis~\ref{item:it2}, using Cauchy sequences. Their equality is not immediate.
%By Hypothesis~\ref{item:it1} and the formula $C(f):=\Upsilon(f)-|\alpha(f)|\Upsilon(\cal R(f))$ it amounts to proving that $\Upsilon(f_0 \circ R_\alpha)$ has left and right limits that are equal. This was proved
For Hypothesis~\ref{item:it2}, recall that we proved in Proposition~\ref{prop:samelim} that $\alpha\mapsto\Upsilon(f_0\circ R_{\alpha})$ has left and right limits at $0$ that are equal. Since $\Upsilon$ is bounded (Hypothesis~\ref{item:it1}) and $C(f):=\Upsilon(f)-|\alpha(f)|\Upsilon(\cal R(f))$, it follows that $\alpha\mapsto C(f_0\circ R_{\alpha})$ also has left and right limits at $0$ that are equal.
Then:
\bEA C(f)-C(g) & = & \phantom{+}\,C(f)-\lim_{\alpha \underset{<}\to 0} C(f_0 \circ R_\alpha)  
\\ & & + \lim_{\alpha \underset{<}\to 0} C(f_0 \circ R_\alpha) - \lim_{\alpha \underset{>}\to 0} C(f_0 \circ R_\alpha)
\\ & & + \lim_{\alpha \underset{>}\to 0} C(f_0 \circ R_\alpha) - C(f_0\circ R_{\alpha(g)}) 
\\ & & + \, C(f_0\circ R_{\alpha(g)})-C(g).\eEA
Recall that $d_{\log}(f,g) := d_{\log}(\alpha(f),\alpha(g)) + d_T(f_0,g_0)$. 
By the case when both rotation numbers are negative, we know that for $\alpha\in (\alpha(f),0)$,
$|C(f)-C(f_0\circ R_\alpha)| \leq K_1 d_{\log}(f, f_0\circ R_\alpha)=0+ K_1 d_{\log}(\alpha(f),\alpha)$. Thus by passing to the limit $\alpha\underset{<}\tend 0$, we get that the first term in the sum above is $\leq K_1 d_{\log}(\alpha(f),0)$. Similarly, the third is $\leq K_1 d_{\log}(0,\alpha(g))$. We have proved that the second term is null. For the fourth term, by the case when both rotation numbers are positive, we get $|C(f_0\circ R_{\alpha(g)})-C(g)| \leq K_1 d_{\log}(f_0\circ R_{\alpha(g)},g) = K_1 d_T(f_0,g_0)+0$. All in all:
$|C(f)-C(g)| \leq K_1\big( d_{\log}(\alpha(f),0)+ d_{\log}(0,\alpha(g)) + d_T(f_0,g_0)\big)$. Since $\alpha(f)$ and $\alpha(g)$ have opposite signs, $d_{\log}(\alpha(f),0)+ d_{\log}(0,\alpha(g)) = d_{\log}(\alpha(f),\alpha(g))$. 
Whence $|C(f)-C(g)| \leq K_1 d_{\log}(f,g)$.
\end{proof}

Under the above hypotheses, we will prove:

\begin{thm}\label{thm:map}
 $\exists A,B>0$ such that $\forall f,g \in \IS_N$,
\[|\Upsilon(f)-\Upsilon(g)| \leq A\,d(\alpha(f),\alpha(g))^{1/2} + B\, d(f_0,g_0)\]
and $\forall \alpha,\beta\in \HT_N$,
\[|\Upsilon(P_\alpha)-\Upsilon(P_\beta)| \leq A\,d(\alpha(f),\alpha(g))^{1/2}.\]
\end{thm}

\begin{rem}
As previously noted, the (uniform) modulus of continuity of $\Upsilon$ with respect to the rotation number will not be better than $1/2$-H\"older. However, the pointwise modulus of continuity can be better at some values. Note that since H\"older continuous maps are uniformly continuous, $\Upsilon$ extends to the closure of $\HT_N$, which consists of $\HT_N$ plus some rationnals. Let $x$ be one of them (for instance, $x=0$). Then with a finite number of renormalizations, it follows from the continuity of $\Upsilon$, and the above hypotheses that $\Upsilon$ has a modulus of continuity at $x\in\Q$ of the form: 
\[|\Upsilon(x+\epsilon)-\Upsilon(x)| \leq c_x \big|\epsilon\log|\epsilon|\big|
\]
(in a neighborhood of $x$). This is much better than $|\epsilon|^{1/2}$, almost as good as $|\epsilon|$. However, $c_x$ depends on $x$.
It cannot be better than $\big|\epsilon\log|\epsilon|\big|$, though: from~\cite{HDR08}, we know that, for quadratic polynomials, at rationals $x$ and for some well chosen subsequences $\epsilon_n\tend 0$, the function $\Upsilon$ has expansion of the form $\Upsilon(x+\epsilon_n) = a_x + b_x\epsilon_n \log |\epsilon_n| + c_x \epsilon_n + o(\epsilon_n)$.
\end{rem}



\subsection{Discussion about rotation number one half}

The Marmi Moussa Yoccoz conjecture concerns a function $\Upsilon$ that is defined on the 1-torus $\R/\Z$ (or it can be viewed as a $1$-periodic function on $\R$).
Recall the number $N\geq$ involved in the definition of high type numbers (using modified continued fractions).
Note that for $N=2$, the high type numbers are all the irrationals! In $\R/\Z$, the set of high type numbers is bounded away from $1/2$ as soon as $N\neq 2$.
According to discussion with them, the number $N$ provided by Inou and Shishikura is likely to be no less than $20$.
However, it is widely believed that a modification of their construction would work for all rotation numbers.
But extra caution should be taken near rotation number $1/2$: indeed, it is known that as $\alpha$ varies from $0$ to $1/2$, the fundamental cylinders used in parabolic renormalization tend to different domains as when $\alpha$ varies from $0$ to $-1/2$.
But in $\R/\Z$, $-1/2=1/2$. \emph{This means that there is a discontinuity of cylinder renormalization as one crosses $1/2$.}
To solve this, we believe one should use an extension of one of the two branches of the renormalization operator beyond $1/2$. However, in the present article, we will not worry with that and we will assume $N\geq 3$. We will work in $\R$ instead of $\R/\Z$ and make statements about $\HT_N\cap [-1/2,1/2]$.

\begin{rem}
Crossing $0$ also creates problems and a discontinuity of the renormalization operator, but sizes get multiplied by a factor tending to $0$, which absorbs the discontinuity: this is used in the proof of hypothesis~\ref{item:it2} in Section~\ref{subsec:map}.
\end{rem}

\subsection{Proof, first steps}

The proof of Theorem~\ref{thm:map} is split across the remaining subsections of Section~\ref{sec:arn}.

\bigskip

For $f\in\cal IS_\R$ let $\cal S(f) = f$ if $\alpha(f) \in[0,1/2]$ and $\cal S(f) = s\circ f\circ s$ otherwise, where $s(z)=\ov z$.
It is defined so that the rotation number of $(\cal{SR})^n(f)$ coincides with the sequence $\alpha_n(f)$ associated to the modified continued fraction of $\alpha(f)$.
To shorten the notations in subsequent computations, we will denote
\[f_n = (\cal {SR})^n(f)\text{ and }g_n = (\cal {SR})^n(g).\]
It is important to note that $\cal S$ is not continuous with respect to $f$ as $\alpha(f)$ crosses $0$. Hence an inequality like Hypothesis~\ref{item:it4} cannot hold with $(\cal{SR})_0$ replacing $\cal R_0$.
Note also that
\[Y(-\alpha) = Y(\alpha),\quad r(\cal S f)=r(f),\quad \Upsilon(\cal Sf)=\Upsilon(f)\]
thus
\[C(f) = \Upsilon(f)-|\alpha(f)|\Upsilon(\cal{SR}(f)).\]


Let $f\in\IS_N\cup \Pol_N$. Then for all $n>0$, $f_n\in\IS_N$.
By induction for all $n\in\N$,
\[\Upsilon(f) = \sum_{k=0}^{n} \beta_{k-1}(f) C(f_k) + \beta_n(f)\Upsilon(f_{n+1}).\]
Let $n\tend+\infty$. Since $\beta_n(f)\tend 0$, and $\Upsilon$ is bounded over $\IS_N$, we get
\[\Upsilon(f) = \sum_{k=0}^{+\infty} \beta_{k-1}(f) C(f_k),\]
which is by itself an interesting formula.

Now assume either $f,g \in \IS_N$ or $f,g\in \Pol_N$: if $\alpha(f)=\alpha(g)$ then denoting $\beta_k=\beta_k(f)=\beta_k(g)$,
\[\Upsilon(f)-\Upsilon(g)  =  \sum_{k=0}^{+\infty} \beta_{k-1}(f) \big(C(f_k) - C(g_k)\big),\]
whence
\begin{equation}\label{eq:upup1} \big|\Upsilon(f)-\Upsilon(g)\big|  \leq  K_1\sum_{k=0}^{+\infty}\beta_{k-1}\,d_{\log}(f_k,g_k).
\end{equation}
Otherwise, 
let us split the summand the usual way:
\bEA
\beta_{k-1}(f) C(f_k) - \beta_{k-1}(g) C(g_k) & = &
\beta_{k-1}(f) C(f_k) - \beta_{k-1}(f) C(g_k)
\\ &+  & \beta_{k-1}(f) C(g_k) - \beta_{k-1}(g) C(g_k) .
\eEA
Hence
\bEA
\big|\beta_{k-1}(f) C(f_k) - \beta_{k-1}(g) C(g_k)\big| & \leq &
\beta_{k-1}(f) \times \big| C(f_k) - C(g_k)\big|
\\ & + & \big|\beta_{k-1}(f) - \beta_{k-1}(g)\big| \times |C(g_k)|.
\eEA
Whence
\begin{equation}\label{eq:upup}
\big| \Upsilon(f)-\Upsilon(g) \big|  \leq \sum_{k=0}^{+\infty}\beta_{k-1}(f)\,|C(f_k)-C(g_k)| + K_3\sum_{k=0}^{+\infty}|\beta_{k-1}(f)-\beta_{k-1}(g)|.
\end{equation}

\subsection{First term}\label{subsec:firstterm}

Here we deal with the term 
\[\sum_{k=0}^{+\infty}\beta_{k-1}(f)\,|C(f_k)-C(g_k)|.\]
To shorten the notations we let $\alpha = \alpha(f)$, $\alpha' = \alpha(g)$, $\alpha_n$ and $\beta_n$ associated to $\alpha$,  $\alpha'_n$ and $\beta'_n$ associated to $\alpha'$ and
\[ d'_n = d_{\log}(\alpha_n,\alpha'_n) % \left|\int_{\alpha_n}^{\alpha'_n} \bigl|\log |x|\bigr|dx\right|
.\]
Let $n_0\geq 0$ be \emph{the first integer so that $\alpha_{n_0}(f)$ and $\alpha_{n_0}(g)$ belong to different fundamental intervals}.
For some values of $k$ we will use $|C(f_k)-C(g_k)|\leq K_1 d_{\log}(f_k,g_k)$.
Recall that either $f,g\in\IS_N$ or $f,g\in\Pol_N$. In the second case we set $d_T((f)_0,(g)_0)=0$. Then:
\begin{itemize}
\item for $k=0$, $d_{\log}(f_k, g_k) = d_{\log}(f,g) = d_T((f)_0,(g)_0) + d'_0$,
\item for $1\leq k\leq n_0$, $d(( f_k)_0,(g_k)_0) \leq  \lambda d((f_{k-1})_0,(g_{k-1})_0) + K_2 d'_{k-1}$
\item thus by induction: for $0\leq k\leq n_0$,
\[ d(( f_k)_0,( g_k)_0) \leq \lambda^k d_T((f)_0,(g)_0) + K_2 \sum_{m=0}^{k-1} \lambda^{k-1-m} d'_m
,\]
whence
\[ d_{\log}( f_k, g_k) \leq \lambda^k d_T((f)_0,(g)_0) + K_2 \sum_{m=0}^{k-1} \lambda^{k-1-m} d'_m + d'_k 
.\]
\item $d((\cal R f_{n_0})_0,(\cal R g_{n_0})_0) \leq  \lambda d((f_{n_0})_0,(g_{n_0})_0) + K_2 d'_{n_0}$
\end{itemize}
Then
\bEA
\sum_{k=0}^{n_0}\beta_{k-1}\,d_{\log}(f_k,g_k) \leq  \left(\sum_{k=0}^{n_0} \beta_{k-1}\lambda^k\right) d_T(f_0,g_0) +
 & & \\
K_2\sum_{k=0}^{n_0} \beta_{k-1} \sum_{m=0}^{k-1} \lambda^{k-1-m}d'_m + \sum_{k=0}^{n_0} \beta_{k-1} d'_k.
\eEA
Let us regroup the terms according to $d'_0$, $d'_1$, $d'_2$, \ldots:
\bEA
\sum_{k=0}^{n_0}\beta_{k-1}\,d_{\log}(f_k,g_k) \leq  \left(\sum_{k=0}^{n_0} \beta_{k-1}\lambda^k\right) d_T(f_0,g_0) +
 & & \\
\sum_{j=0}^{n_0}  d'_j \left(\beta_{j-1}+K_2\sum_{k=j+1}^{n_0} \beta_{k-1} \lambda^{k-1-j}\right)
.\eEA
Note that since $\lambda<1$ and $\beta_{k-1}\leq 1/2^k$, we get $\sum_{k=0}^{n_0} \beta_{k-1}\lambda^k \leq 2$.
Let us bound the following factor in the preceding estimate:
\bEA
& & \beta_{j-1}+K_2\sum_{k=j+1}^{n_0} \beta_{k-1} \lambda^{k-1-j} \\
& \leq & \beta_{j-1}+K_2\sum_{k=j+1}^{+\infty} \beta_{k-1} \lambda^{k-1-j} \\
& = & \beta_{j-1} \left(1+ K_2 \sum_{k=j+1}^{+\infty} \alpha_{j}\cdots \alpha_{k-1} \lambda^{k-1-j} \right) \\
& \leq & \beta_{j-1} \left(1+ K_2 \sum_{j=1}^{+\infty} 2^{-j} \right) \qquad\text{(}\lambda\leq 1 \text{ and }a_j\leq 1/2\text{)}\\
& = & \beta_{j-1} (1+ K_2)
\eEA
Finally we get 
\[ \sum_{k=0}^{n_0}\beta_{k-1}\,|C(f_k)-C(g_k)| \leq 2 K_1\,d_T(f_0,g_0) +K_1(1+K_2)\sum_{j=0}^{n_0}\beta_{j-1}d'_j.
\]
For the remaining terms, we will make two cases:
\begin{enumerate}
\item[(A)] The fundamental intervals $\alpha_{n_0}$ and $\alpha'_{n_0}$ belong to are adjacent and have symbols $(a,+)$, $(a,-)$ with the same value of $a$. 
\item[(B)] The other case.
\end{enumerate}
In case (A) we let $n_2=n_0+2$, in case (B) $n_2=n_0+1$.
If necessary, let us permute\footnote{This permutation is done only at this point of the article, so it is safe.} $f$ and $g$, so that $\alpha_{n_0}>\alpha'_{n_0}$.
\begin{lem}
$|\alpha-\alpha'| \geq e^{-2C} \beta_{n_2-1}^2 /12$.
\end{lem}
\begin{proof}
If the two intervals are not adjacent, then we are in case (B), so $n_2=n_0+1$.  Let $I$ be the first generation interval just left to that containing $\alpha_{n_0}$. Then it separates $\alpha_{n_0}$ from $\alpha'_{n_0}$ thus $\alpha$ and $\alpha'$ are separated by the fundamental interval of generation $n_2$ adjacent to that of $\alpha$ and corresponding under $H_n$ to $I$. By the estimates following Lemma~\ref{lem:bd},
\[ |\alpha-\alpha'|\geq e^{-2C}\beta_{n_2-1}^2/2.\]

If the intervals are adjacent but with symbols $(a,+)$, $(a+1,-)$ we are aslo in case (B). Recall that we assumed $N\geq 3$. There is thus a pair of generation $n_0+2$ intervals $I$ and $I'$ with symbol $(2,+)$ inside $I_{n_0+1}(\alpha)$ and $I_{n_0+1}(\alpha')$ separating $\alpha$ from $\alpha'$. The quotients $|I|/|I_{n_0+1}(\alpha)|$ and $|I'|/|I_{n_0+1}(\alpha')|$ are both bounded from below, using bounded distorsion (Lemma~\ref{lem:bd}), by $e^{-C}$ times the value of this quotient for first generation intervals, which is equal to $1/6$. We have $|\alpha-\alpha'| \geq |I|+|I'|$ but for convenience, let us forget $|I'|$:
\[\alpha-\alpha'\geq e^{-2C}\beta_{n_2-1}^2/12\]

Otherwise, we are in case (A): $n_2=n_0+2$. There is a fundamental interval of generation $n_0+2$ inside $I_{n_0+1}(\alpha)$ that separates $\alpha$ from $\alpha'$. Hence\footnote{This estimate sufficient but is far from optimal. A bound of order $\beta_{n_2-2}^2(\alpha_{n_2-1}+\alpha_{n_2-1})$ can be obtained.}
\[|\alpha-\alpha'| \geq e^{-2C}\beta_{n_2-1}^2/2.\]
\end{proof}
%
In both cases (A) and (B), to bound the part of the sum with $k\geq n_2$, let us use $\beta_{k-1}\,|C(f_k)-C(g_k)| \leq 2K_3\beta_{k-1}$ and
$\sum_{k=n_2}^{+\infty} \beta_{k-1} \leq 2 \beta_{n_2-1}$, whence
\[ \sum_{k=n_2}^{+\infty} \beta_{k-1}\,|C(f_k)-C(g_k)| \leq 4 K_3 \beta_{n_2-1} \leq 4 e^C K_3 \sqrt{12}  |\alpha-\alpha'|^{1/2}.
\]

The only term of the sum that we have not bounded is the one with $k=n_0+1$ in case (A). 
Let $\wt f_{n_0+1} = \cal R f_{n_0}$ (compare with $f_{n_0+1} = \cal{SR}f_{n_0}$) and $\wt g_{n_0+1} = \cal R g_{n_0}$.
Since $C(f)=C(\cal S f)$ for all $f$, this implies that 
\[ |C(f_{n_0+1})-C(g_{n_0+1})| = |C(\wt f_{n_0+1})-C(\wt g_{n_0+1})|
.\]
Similarly, let $\wt \alpha_{n_0+1} = 1/\alpha_{n_0} - a_{n_0+1} \in [-1/2,1/2]$, and $\wt \alpha'_{n_0+1} = 1/\alpha'_{n_0} - a'_{n_0+1} \in [-1/2,1/2]$
This has been chosen so that: $\wt f_{n_0+1}'(0)=e^{2\pi i \wt \alpha_{n_0+1}}$ and $\wt g_{n_0+1}'(0)=e^{2\pi i \wt \alpha'_{n_0+1}}$.
Let us now introduce the intermediary function $h=e^{2\pi i \wt \alpha'_{n_0+1}} (\wt f_{n_0+1})_0$. Then
\[|C(f_{n_0+1})-C(g_{n_0+1})| \leq |C(\wt f_{n_0+1})-C(h)|+|C(h)-C(\wt g_{n_0+1})|
.\]
Then we will use the Lipschitz property of $C$ with respect to $d_{\log}$.
For the term $|C(h)-C(\wt g_{n_0+1})|$, we obtain the upper bound $K_1\big(d_T((h)_0,(\wt g_{n_0+1})_0)+0\big)$, which equals 
$K_1\times0+K_1d_T\big((\wt f_{n_0+1})_0,(\wt g_{n_0+1})_0\big)$. 
For the term $|C(\wt f_{n_0+1})-C(h)|$ we obtain the upper bound $K_1 d_{\log}(\wt \alpha_{n_0+1},\wt\alpha'_{n_0+1})$, which equals $K_1d_{\log}(-\alpha_{n_0+1},\alpha'_{n_0+1})$. Hence
\[|C(f_{n_0+1})-C(g_{n_0+1})| \leq K_1 \Big( d_T\big((\wt f_{n_0+1})_0, (\wt g_{n_0+1})_0\big)+ d_{\log}(-\alpha_{n_0+1},\alpha'_{n_0+1})\Big)
.\]
Now we can use
\[d_T\big((\wt f_{n_0+1})_0,(\wt g_{n_0+1})_0\big) \leq \lambda d_T\big((f_{n_0+1})_0,(g_{n_0+1})_0\big) + K_2 d_{\log}(\alpha_{n_0},\alpha'_{n_0}),\]
thus
\[d_T\big((\wt f_{n_0+1})_0,(\wt g_{n_0+1})_0\big) \leq \lambda^{n_0+1} d_T((f)_0,(g)_0) + K_2 \sum_{m=0}^{n_0} \lambda^{n_0-m} d'_m + d'_{n_0+1}\]
which can be incorporated to the computation made earlier of the sum from $k=0$ to $n_0$. So, in case (A):
\bEA \sum_{k=0}^{n_0+1}\beta_{k-1}\,|C(f_k)-C(g_k)| & \leq & 2 K_1\,d_T(f_0,g_0) +K_1(1+K_2)\sum_{j=0}^{n_0+1}\beta_{j-1}d'_j 
\\ & + & K_1\beta_{n_0} d''_{n_0+1}
\eEA
with $d''_{n_0+1} = d_{\log}(-\alpha_{n_0+1},\alpha'_{n_0+1})$. Let $x$ be the touching point between the generation $n_0+1$ fundamental intervals containing $\alpha$ and $\alpha'$: $|\alpha-\alpha'|=|\alpha-x|+|\alpha'-x|$.
By bounded distorsion (Lemma~\ref{lem:bd}), $|\alpha-x| \geq e^{-C} \beta_{n_0}^2 \alpha_{n_0+1}$.
Similarly (see the discussion following the Lemma~\ref{lem:bd}) $|\alpha'-x| \geq e^{-2C} \beta_{n_0}^2 \alpha'_{n_0+1}$.
So $|\alpha-\alpha'| \geq \beta_{n_0}^2e^{-2C}(\alpha_{n_0+1} +\alpha'_{n_0+1})$. Using now $d_{\log}(-\alpha_{n_0+1},\alpha'_{n_0+1}) \leq M_0(\alpha_{n_0+1} +\alpha'_{n_0+1})^{1/2}$ we get
\[\beta_{n_0} d''_{n_0+1} \leq M_0 e^C |\alpha-\alpha'|^{1/2}.\]

Taking both cases (A) and (B) into account, we get:
\bEA \sum_{k=0}^{+\infty}\beta_{k-1}\,|C(f_k)-C(g_k)| & \leq & M_1 |\alpha-\alpha'|^{1/2} + 2 K_1\,d_T(f_0,g_0)  
\\ & + & K_1(1+K_2) \sum_{j=0}^{+\infty}\beta_{j-1}d'_j
\eEA
where $M_1 = 4e^C K_3\sqrt{12}+K_1 M_0 e^C$.


\subsection{Second term}\label{subsec:secondterm}

Let us now deal with the term 
\[ K_3 \sum_{k=0}^{+\infty}|\beta_{k-1}(f)-\beta_{k-1}(g)|.
\]

\begin{rem} For the modified continued fraction algorithm, each $\beta_k$ is a continuous function of $\alpha$, whereas it is not the case for the classical continued fractions. 
Note also that each $\beta_k$ is in fact $1/2$-H\"older continuous (with respect to $\alpha$) with constant $B_k$, and that the sequence $B_k$ is bounded but unfortunaltely does not tend to $0$, thus $\sum B_k$ is not convergent.
\end{rem}

The computation goes:
\bEA & &
\sum_{k=0}^{+\infty}|\beta_{k-1}(f)-\beta_{k-1}(g)| = \sum_{k=0}^{+\infty}|\beta_{k}(f)-\beta_{k}(g)|
\leq \\ & & 
\sum_{k=0}^{+\infty} \sum_{j=0}^{k} \alpha_0 \cdots \alpha_{j-1} \Big|\alpha_j-\alpha'_j\Big|\alpha'_{j+1} \cdots \alpha'_{k}
= \\ & &
\sum_{j=0}^{+\infty} \alpha_0\cdots\alpha_{j-1}|\alpha_j-\alpha'_j|\sum_{k=j}^{+\infty} \alpha'_{j+1}\cdots\alpha'_{k}
\eEA
%
With the convention that for $k=j$, $\alpha'_{j+1}\cdots\alpha'_{k} = 1$. Since each $\alpha'_i$ is $\leq 1/2$, we get
\[\sum_{k=j}^{+\infty} \alpha'_{j+1}\cdots\alpha'_{k} \leq 2
.\]
Hence, using the following notations:
\[ d_n = |\alpha_n-\alpha_n'|,
\]
we obtain the following bound on the second term:
\bEA & & K_3\sum_{k=0}^{+\infty}|\beta_{k-1}(f)-\beta_{k-1}(g)| + K_0 |\beta_{+\infty}(f)-\beta_{+\infty}(g)|
\\ & & \leq 2\max(K_3,K_0) \sum_{j=0}^{+\infty} \beta_{j-1} d_j
.\eEA


\subsection{Arithmetics}\label{subsec:arith}

\ldots with a strong analytic flavor. The work presented below is not original: it is basically a simplified version of part of~\cite{MMY97}, reformulated in different notations.

\subsubsection{Estimates on the size of fundamental intervals}

As a trick to simplify the presentation of the next section, we introduce \emph{extended fundamental intervals} of generation $n$. These are the sets on which $H_{n+1}$ is continuous. They can also be characterized as the the union of two consecutive fundamental intervals of generation $n$ and their common boundary point, but only for those pairs whose symbols end with respectively $(a_n,+)$ and $(a_n+1,-)$ (the rest of their symbol must be identical). Like the fundamental intervals, their collection also form a nested sequence of partitions of the irrationals. Like above, for $\alpha$ irrationnal, we will denote
\[\wt I_n(\alpha)\]
the $n$-th generation extended fundamental interval containing $\alpha$.
Another corollary of Lemma~\ref{lem:bd} is that for two consecutive fundamental intervals $I,I'$ at a given level, we have:
\[ e^{-2C} \leq \frac{|I'|}{|I|} \leq e^{2C}
.\]
In fact we will use the following slightly better\footnote{The proof could be as well carried out without this improvement} estimate, using the fact that the left derivative and the right derivative of $H_n$, at points where adjacent fundamental intervals meet, have equal absolute values:
\[\forall \alpha\in I,\ e^{-2C} \leq \frac{\big|I'\big|}{\beta_{n-1}^2/2}\leq e^{2C}\]
whence
\begin{equation}\label{eq:iiprime}
\forall \alpha\in I,\ e^{-C}+e^{-2C} \leq \frac{|\wt I_n(\alpha)|}{\beta_{n-1}^2/2}\leq e^{C}+e^{2C}.
\end{equation}

More generally, if one has $k$ consecutive adjacent fundamental intervals of generation $n$, and $\alpha$ belongs to one of them, then
the sum $\Sigma$ of their lengths satisfies
\[ e^{-C}+e^{-2C}+\cdots+e^{-kC}\leq \frac{ \Sigma}{\beta_{n-1}^2/2}\leq e^C+e^{2C}+\cdots+e^{kC}
.\]

Let us now try and give various estimates of $|\alpha-\alpha'|$ in terms of their modified continued fraction expansion.
Assume that $\alpha,\alpha'\in[-1/2,1/2]$, that they are both irrationals and that $\alpha\neq \alpha'$. Let $n\geq 0$ be the first integer such that $\alpha$ and $\alpha'$ do not belong to the same generation $n$ extended fundamental interval.
If $n>0$, from $\wt I_{n_1-1}(\alpha)= \wt I_{n-1}(\alpha')$ we get the upper bound $|\alpha-\alpha'| \leq |\wt I_{n-1}(\alpha)| $ thus
\[|\alpha-\alpha'| \leq \frac{e^{C}+e^{2C}}{2} \beta_{n-2}^2.\]
Depending on the situations, this upper bound can be far from sharp. 
For a lower bound, let us consider the two cases: %\comment{bien faire attention au cas $n=0$}
\begin{itemize}
\item If $\wt I_n(\alpha)$ and $\wt I_n(\alpha')$ are not adjacent, then
\[ \frac{e^{-2C}+e^{-3C}}{2} \beta_{n-1}^2 \leq |\alpha-\alpha'| 
.\]
\item If they are adjacent, then
\[  e^{-4C} (\alpha_n+\alpha'_n)\beta_{n-1}^2 \leq |\alpha-\alpha'| % \leq (e^C+e^{2C}+e^{3C}+e^{4C})\beta_{n-1}^2/2
.\]
\end{itemize}
Those estimates can also be far from optimal.
\begin{proof}
In the first case, $\alpha$ and $\alpha'$ are separated by at least one extended interval adjacent to the one containing $\alpha$.

In the second case, $[\alpha,\alpha']$ intersects between $2$ and $4$ fundamental intervals (on which $H_n$ is a bijection). Let $u$ be the common point in the boundaries of $\wt I_n$ and $\wt I_n'$.
Then $[\alpha,\alpha']\setminus \{u\}$ splits into two components: $[\alpha,u)\subset \wt I_n$, and $(u,\alpha']\subset \wt I'_n$. 
Consider $[\alpha,u)$. Then it is either contained in only one fundamental interval, in which case it is equal to the connected component $J$ containing $\alpha$ of $H_n^{-1}((0,\alpha_{n}))$, and $|J| \geq e^{-C}\beta_{n-1}^{-2} \alpha_n$.
Or it is not and then it contains the component $J$ of $H^{-1}((0,1/2))$ that is contained in $\wt I_n$, and $|J|\geq e^{-2C} \beta_{n-1}^{-2} /2$. In both cases, $|J| \geq e^{-2C}\beta_{n-1}^{-2}\alpha_n$. Similarly, $(u,\alpha']$ contains an interval $J'$ whose length is $\geq e^{-4C}\beta_{n-1}^{-2}\alpha'_n$. 
Now $|\alpha-\alpha'|\geq |J|+|J'| \geq (e^{-2C}\alpha_n+e^{-4C}\alpha'_n)\beta_{n-1}^2 \geq e^{-4C}(\alpha_n+\alpha'_n)\beta_{n-1}^2$, thus we get the lower bound 
$e^{-4C}(\alpha'_n+\alpha_{n})\beta_{n-1}^2
 \leq |\alpha-\alpha'|$.
The upper bound follows from the remark after Equation~\ref{eq:iiprime}.
\end{proof}
Note that in the two cases, we get the following weaker lower bound:
\begin{equation}\label{eq:wlb} 2e^{-4C}\beta_{n}^2 \leq |\alpha-\alpha'|
.\end{equation}

\subsubsection{Bounding an arithmetically defined sum}\label{sss:bads}


The work of Sections~\ref{subsec:firstterm} and~\ref{subsec:secondterm}, to prove the main theorem, we are reduced to bound the quantities $\sum_{j=0}^{+\infty} \beta_{j-1} d'_j$ and $\sum_{j=0}^{+\infty} \beta_{j-1} d_j$ by constants times $|\alpha-\alpha'|^{1/2}$. Since $d'_j>d_j$, it is enough to bound the first sum. Note that $\forall x,y\in[-1/2,1/2]$,
\[d_{\log}(x,y)\leq M_a |x-y|^a.\]
This follows for instance from H\"older's inequality, or more simply from the following computation:
if $x,y$ of the same sign then $\big|\int_x^y dt/|t|\big| \leq \int_0^{|x-y|} dt/t$, if $x,y$ have opposite sign then $\big|\int_x^y dt/|t|\big| \leq 2\int_0^{|x-y|/2} dt/t$. It implies in particular, for all $a\in(0,1)$, 
\[d'_j \leq M_a |\alpha_j-\alpha'_j|^a\]
where $M_a$ depends only on $a$.
The first term of the sum to be bounded is $\beta_{-1}d'_0 = 1\times d_{\log}(\alpha,\alpha')$. Applying the above with $a=1/2$, we see that it is enough to bound the sum over $j\geq1$. Choose your preferred $a\in(0,1/2)$, for instance $a=1/4$. By the discussion above, the following lemma is sufficient to conclude the proof of the main theorem.

\begin{lem} Let $a\in(1/2,1)$. There exists $K>0$, which depends on $a$, such that $\forall \alpha,\alpha' \in [-1/2,1/2]$ that are irrational,
\[\sum_{j=1}^{+\infty} \beta_{j-1} |\alpha_j-\alpha'_j|^a \leq K |\alpha-\alpha'|^{1/2}
.\]
\end{lem}
\begin{rem} Marmi, Moussa and Yoccoz realized that we cannot get a better exponent on the right hand side.
They also noted that taking $a\in (0,1/2)$ gives a function which is $a$-H\"older (Theorem~4.2 in~\cite{MMY97} with $\nu=1$ and $\eta=a$).
\end{rem}
\begin{proof}

Assume $\alpha\neq\alpha'$ for otherwise the  sum is $0$. As in Section~\ref{sec:mcf}, let $n\geq 0$ be the first integer for which $\alpha$ and $\alpha'$ belong to different extended fundamental intervals of generation $n$.
Let $j\geq 1$. To bound $\beta_{j-1} |\alpha_j-\alpha'_j|^a$ we will consider different cases.

\smallskip\noindent\textbf{Case 1, $j<n$:} If $j\leq n-2$, then $\alpha$ and $\alpha'$ lie in the same $j$-th generation fundamental interval.
By bounded distorsion of $H_j:\alpha\mapsto \alpha_j$ on fundamental intervals, $|\alpha_j-\alpha'_j| \leq e^{C} H_j'(\alpha) |\alpha-\alpha'| = e^{C} \beta_{j-1}^{-2} |\alpha-\alpha'|$.
For $j=n-1$, $\alpha$ and $\alpha'$ lie in the same $j$-th generation extended fundamental interval, whence $|\alpha_j-\alpha'_j| \leq e^{2C} \beta_{j-1}^{-2} |\alpha-\alpha'|$. In both cases, i.e.\ for all $j\leq n-1$, we have
\[|\alpha_j-\alpha'_j| \leq e^{2C} \beta_{j-1}^{-2} |\alpha-\alpha'|.\]
Recall that $|\alpha-\alpha'| \leq (e^C+e^{2C})\beta_{n-2}^2/2$, thus
\bEA
& \ds \frac{\beta_{j-1}|\alpha_j-\alpha'_j|^a}{|\alpha-\alpha'|^{1/2}}
\leq e^{2Ca}\left(\frac{|\alpha-\alpha'|}{\beta_{j-1}^{2}}\right)^{a-1/2}
\leq  K_4\left(\frac{\beta_{n-2}}{\beta_{j-1}}\right)^{a-1/2} \ =
& \\  & \ds =\ K_4 (\alpha_{j} \cdots \alpha_{n-2})^{a-1/2}\ \leq\ K_4\left(\frac{1}{2^{(n-1)-j}}\right)^{a-1/2}
. & \eEA
With $K_4 = e^{2Ca} \left(\frac{e^C+e^{2C}}{2}\right)^{a-1/2}$ and the convention that $\alpha_{j} \cdots \alpha_{n-2}=1$ if $j=n-1$.
 Whence
\[ \beta_{j-1}|\alpha_j-\alpha'_j|^a \leq \frac{K_4}{u^{n-1-j}} |\alpha-\alpha'|^{1/2}
\]
with $u=2^{a-1/2}>1$.

\smallskip\noindent\textbf{Case 2, $j > n$:} Then $|\alpha_j-\alpha_j'| \leq 1/2 < 1$ and $\beta_{j-1} = \alpha_0 \cdots \alpha_{j-1} = \beta_{n} \alpha_{n+1} \cdots \alpha_{j-1} \leq \beta_{n} /2^{j-n-1} \leq \frac{e^{2C}}{\sqrt{2}} |\alpha-\alpha'|^{1/2} /2^{j-n-1}$ by Equation~\eqref{eq:wlb}. Whence
\[\beta_{j-1}|\alpha_j-\alpha'_j|^a \leq \frac{K_5}{2^{j-(n+1)}} |\alpha-\alpha'|^{1/2}\]
with $K_5 = e^{2C}\sqrt{2}$.

\smallskip\noindent\textbf{Case 3, $j=n$:} We consider two sub-cases:
\begin{itemize}
\item $\wt I_n$ and $\wt I_n'$ are not adjacent. Then starting from 
$|\alpha_n-\alpha'_n| \leq 1/2<1$ and $|\alpha-\alpha'|\geq (e^{-2C}+e^{-3C})\beta_{n-1}^2/2$, 
we get 
\begin{gather*}
\beta_{n-1}|\alpha_n-\alpha'_n|^a / |\alpha-\alpha' |^{1/2} \leq  \sqrt{2/(e^{-2C}+e^{-3C})}\\
\beta_{n-1}|\alpha_n-\alpha'_n| \leq K_6 |\alpha-\alpha'|^{1/2}
\end{gather*}
with $K_6 = \sqrt{2/(e^{-2C}+e^{-3C})}$.
\item $\wt I_n$ and $\wt I_n'$ are adjacent. 
Then starting from 
\[|\alpha_n-\alpha'_n| \leq 1/2 <1 \tand e^{-4C}(\alpha'_n+\alpha_{n})\beta_{n-1}^2 \leq |\alpha-\alpha'|\]
we get
\[
\ds \beta_{n-1}|\alpha_n-\alpha'_n|^a / |\alpha-\alpha'|^{1/2} \leq e^{2C}\frac{|\alpha_n-\alpha'_n|^a}
{\sqrt{\alpha_n+\alpha'_n}}.\] 
Now $|\alpha_n-\alpha'_n|\leq \max(\alpha_n,\alpha'_n)$ and $\alpha_n+\alpha'_n \geq \max(\alpha_n,\alpha'_n)$ 
thus
\[\ds \beta_{n-1}|\alpha_n-\alpha'_n|^a / |\alpha-\alpha'|^{1/2} \leq e^{2C} \frac{\max(\alpha_n,\alpha'_n)^a}{\sqrt{\max(\alpha_n,\alpha'_n)}} = e^{2C} \left(\max(\alpha_n,\alpha'_n)\right)^{a-1/2} \leq e^{2C}.
\]
\[ \beta_{n-1}|\alpha_n-\alpha'_n|^a \leq K'_6 |\alpha-\alpha'|^{1/2}
\]
with $K'_6 = e^{2C}$.
\end{itemize}

\medskip

\noindent By the first case:
\[\sum_{j=1}^{n-1}\beta_{j-1}|\alpha_j-\alpha'_j|^a \leq K_4\, |\alpha-\alpha'|^{1/2} \sum_{s=0}^{+\infty} \frac{1}{u^s}\]
with $u=2^{a-1/2}>1$.
By the second case:
\[\sum_{j=n+1}^{+\infty}\beta_{j-1}|\alpha_j-\alpha'_j|^a \leq K_5\, |\alpha-\alpha'|^{1/2} \sum_{s=0}^{+\infty} \frac{1}{2^s}.\]
Using the three cases altogether we thus get:
\[ \sum_{j=1}^{+\infty}\beta_{j-1}|\alpha_j-\alpha'_j|^a \leq K_7\,|\alpha-\alpha'|^{1/2}
\]
with $K_7 = \frac{K_4}{1-u}+2K_5+\on{max}(K_6,K'_6)$.
\end{proof}

This proves the lemma, which was the last step to get the theorem.

